$\mathcal{H}_2$-Optimal Model Reduction Using Projected Nonlinear Least Squares

In many applications throughout science and engineering, model reduction plays an important role replacing expensive large-scale linear dynamical systems by inexpensive reduced order models that capture key features of the original, full order model. One approach to model reduction finds reduced order models that are locally optimal approximations in the $\mathcal{H}_2$ norm, an approach taken by the Iterative Rational Krylov Algorithm (IRKA) among others. Here we introduce a new approach for $\mathcal{H}_2$-optimal model reduction using the projected nonlinear least squares framework previously introduced in [J. M. Hokanson, SIAM J. Sci. Comput. 39 (2017), pp. A3107--A3128]. At each iteration, we project the $\mathcal{H}_2$ optimization problem onto a finite-dimensional subspace yielding a weighted least squares rational approximation problem. Subsequent iterations append this subspace such that the least squares rational approximant asymptotically satisfies the first order necessary conditions of the original, $\mathcal{H}_2$ optimization problem. This enables us to build reduced order models with similar error in the $\mathcal{H}_2$ norm but using far fewer evaluations of the expensive, full order model compared to competing methods. Moreover, our new algorithm only requires access to the transfer function of the full order model, unlike IRKA which requires a state-space representation or TF-IRKA which requires both the transfer function and its derivative. Applying the projected nonlinear least squares framework to the $\mathcal{H}_2$-optimal model reduction problem open new avenues for related model reduction problems.

==> alg_lsra.tex <==
\begin{algorithm}[t]
\begin{minipage}{\linewidth}
\begin{algorithm2e}[H]
\Input{Starting poles $\ve\lambda\in \C^r$, $r$ even, weighting matrix $\ma M \in \C^{n\times n}$}
\Output{Pole residue rational approximation $H_r$}
Find ordering $\set I$ minimizing $|\lambda_k - \conj{\lambda_{\set I[k]}}|$ using the Gale-Shapley algorithm\;
Ensure poles come in conjugate pairs $\lambda_k \leftarrow (\lambda_k + \conj{\lambda_{\set I[k]}})/2$\;
Convert poles $\ve\lambda$ into coefficients $\ve b$ such that \cref{eq:quadpartial} has poles $\ve\lambda$\;
\For{$\ell=1,2,3,\ldots$}{
	Compute residual and Jacobian $\uve r, \uma J$ at $\ve b$ \;
	Compute Gauss-Newton step: $\ve d \leftarrow \uma J^+ \uve r$\;
	Set slope $\alpha \leftarrow \ve d^\trans \uma J^\trans \uve r$\;
	\For{$t=\gamma^0, \gamma^1,\ldots$}{
		Compute residual $\uve r_+$ at $\ve b_+ \leftarrow \ve b + t \ve d$\;
		\lIf{$\|\uve r_+\|\le \|\uve r\|_2 + \alpha \beta$}{{\bf break}}
	}
	Update $\ve b \leftarrow \ve b_+$\;
}
Convert rational approximation \cref{eq:quadpartial} to pole residue form\; 
\Function{Residual Jacobian $(\ve b)$}{
	$\ma \Omega \leftarrow
		\ma M^{-1/2}
		\begin{bmatrix}
			\ldots &
			\diag(\ve \mu^2 + b_{2k} \ve\mu + b_{2k-1})^{-1}
			\begin{bmatrix}
				\ve\mu & \ve 1
			\end{bmatrix}
			& 
			\ldots
		\end{bmatrix}
	$\;
	$\uma \Omega \leftarrow \begin{bmatrix} \Re \ma \Omega \\ \Im \ma \Omega \end{bmatrix}$\;
	Set $\uve h \leftarrow \begin{bmatrix} \Re \ma M^{-1/2} \ve H_r \\ \Im \ma M^{-1/2} \ve H_r  \end{bmatrix}$\;
	Compute short form QR decomposition $\uma Q \uma R \leftarrow \uma \Omega$\;
	Compute residual $\uve r \leftarrow \uve h - \uma Q \uma Q^* \uve h$\;
	Compute numerator coefficients $\ve a \leftarrow \uma R^{-1} \uma Q^\trans \uve h$\;
	Form empty Jacobian $\uma J \in \R^{2n \times r}$\;
	\For{$j = 1,2,\ldots, r$}{
		$k \leftarrow \lfloor (j+1)/2 \rfloor$\;
		\If{$j$ is odd}{
			$\partial \ma \Omega \leftarrow -
				\ma M^{-1/2} \diag(\ve\mu^2 + b_{2k} \ve\mu+ b_{2k-1} \ve 1)^{-2}
				\begin{bmatrix} \ve\mu & \ve 1 \end{bmatrix}
			$
		}
		\Else{
			$\partial \ma \Omega \leftarrow -
				\ma M^{-1/2} \diag(\ve\mu) \diag(\ve\mu^2 + b_{2k} \ve\mu+ b_{2k-1} \ve 1)^{-2}
				\begin{bmatrix} \ve\mu & \ve 1 \end{bmatrix}
			$
		}
		$\partial \uma \Omega \leftarrow \begin{bmatrix} \Re \uma \Omega \\ \Im \uma \Omega \end{bmatrix}$\;
		$\uma L \leftarrow -(\ma I - \uma Q \uma Q^\trans) \partial \uma \Omega \ve a$\;
		$\uma K \leftarrow -\uma Q \uma R^{-\trans} \partial \uma \Omega \uve r$\;
		$[\uma J]_{\cdot, j} \leftarrow \uma L +\uma K$\;
	}		
}
% set $k\leftarrow 1$\;
%\For{$\lambda \in \ve \lambda$ with complex $\lambda$ first}{
%	\uIf{$\Im \lambda \ne 0$}{
%		Remove $\lambda$ and $\conj\lambda$ from $\ve\lambda$\;
%		$b_{2k} \leftarrow -2\Re\lambda$\;
%		$b_{2k-1} \leftarrow (\Im\lambda)^2 + (\Re\lambda)^2$\; 
%	}
%	\uElseIf{At least 2 entries in $\ve\lambda$ left}{
%		pick nearest $\lambda'$ in $\ve\lambda$ and remove both $\lambda$ and $\lambda'$ from $\ve\lambda$\;
%		$b_{2k} \leftarrow -(\lambda + \lambda')$\; 
%		$b_{2k-1}\leftarrow -( (\lambda - \lambda') - b_{2k})/4$\;
%	}
%	\uElse{
%		$b_{2k-1} \leftarrow \lambda$\;
%	}
%	$k \leftarrow k +1$\;
%}
\end{algorithm2e}
\vspace{-1em}
\end{minipage}
\caption{Least Squares Rational Approximation}
\label{alg:lsra}
\end{algorithm}


==> background_v0.tex <==
\section{Background}
	Approximation in $\Htwo$ has been popular in engineering applications for several decades.
	Rational Krylov spaces allow for Hermite interpolation of the transfer functions; however, the necessary conditions for optimality were originally posed by Meier and Luenberger without a process to find ROMs that satisfies these conditions.

\subsection{Meier-Luenberger Necessary Conditions for \texorpdfstring{$\Htwo$}{H2} Optimality}

	The following theorem shows that locally optimal approximations with respect to the $\Htwo$ norm satisfy are Hermite interpolants at the reflections of the reduced-order poles across the origin.

	\begin{theorem}[Meier, Luenberger '67]
		Let $H_r$ denote a local minimizer to the optimization problem
		\vspace{-0.5em}
		$$\min_{\substack{H_r \in \Htwo\\ \mbox{deg}(H_r) = r}} \| H - H_r \|_{\Htwo} \vspace{-0.5em}$$
		with distinct poles $\{\lambda_i\}_{i=1}^r$. Then $H_r$ is necessarily a Hermite interpolant of $H$:
		\begin{align}
			\label{eq:ML}
			H(-\lambda_i) = H_r(-\lambda_i), \qquad H'(-\lambda_i) = H_r'(-\lambda_i), \qquad i = 1, \ldots, r.
		\end{align}
	\end{theorem}

	Note that the locally optimal approximation $H_r$ satisfies Hermite interpolation conditions at the reflection of poles of $H_r$, a quantity that unknown until the optimal system is already determined.
	Hence, finding ROM transfer functions $H_r$ that satisfy \eqref{eq:ML} was an unsolved problem until the introduction of IRKA in 2008 \cite{GAB08}.

\subsection{Iterative Rational Krylov Algorithm}

	Gugercin et al.\ introduced the Iterative Rational Krylov Algorithm (IRKA) which was the first method available to find locally optimal $\Htwo$ approximations \cite{GAB08}.
	IRKA was the first algorithm to find reduced-order transfer functions $H_r$ that satisfy the Meier-Luenberger necessary conditions \eqref{eq:ML}.
	
	The algorithm is a Petrov-Galerkin approximation on the FOM $H$, where $\ma A_r = \ma W^T \ma A \ma V$, $\ma B_r = \ma W^T \ma B$, $\ma C_r = \ma C \ma V$. The trial and test spaces $\mathcal V, \mathcal W$ are Rational Krylov spaces with shifts at the Hermite interpolation points $\{\mu_i\}_{i=1}^r$,
	\begin{align}
		\label{eq:RatKrylovSubspace}
		\mathcal V &= \Range(\ma V) = \mbox{span}\{[\mu_1 \ma I - \ma A]^{-1} \ve b, \ldots,  [\mu_r \ma I - \ma A]^{-1} \ve b \},\\
		\mathcal W &= \Range(\ma W) = \mbox{span}\{[\mu_1 \ma I - \ma A]^{-*} \ve c, \ldots,  [\mu_r \ma I - \ma A]^{-*} \ve c \}.
	\end{align}
	
	\noindent When $\ma V, \ma W \in \R^{n\times r}$ then the ROM system $H_r$ is a Hermite interpolant of $H$ at $\{\mu_1,\ldots,\mu_r\}$,
	\begin{align*}
		H(\mu_i) = H_r(\mu_i), \qquad, H'(\mu_i) = H_r'(\mu_i), \qquad i = 1,\ldots, r.
	\end{align*}

	IRKA determines the optimal interpolation points $\{\mu_1,\ldots,\mu_r\}$ by an iterative fixed point algorithm,
	\begin{align}
		\label{eq:IRKA_prog}
		\min_{\ve \mu \in \C^r} \| H(\cdot) - H_r(\cdot;\ve \mu) \|_{\Htwo}^2,
		\qquad
		H_r(\mu_i;\ve\mu) = H(\mu_i),
		\qquad
		H_r'(\mu_i;\ve\mu) = H'(\mu_i).
	\end{align}
	
	The interpolation points $\{\mu_1,\ldots,\mu_r\}$ are chosen via an iterative procedure to find local minimizers of \eqref{eq:IRKA_prog} by the fixed point iteration
	\begin{align*}
		\{\mu_1,\ldots,\mu_r\} \leftarrow \ve\lambda(H_r).
	\end{align*}
	The algorithm is terminated when the interpolation points $\{\mu_1,\ldots,\mu_r\}$ converge to the reflections of the reduced order poles satisfying the Meier-Luenberger necessary conditions \eqref{eq:ML}.
	
	The dominant cost of IRKA is the computation of the Rational Krylov spaces $[\mu_i \ma I - \ma A]^{-1} \ve b$ where $\ma A \in \R^{n\times n}$ and $\ve b \in \R^n$ with $n$ potentially very large.
	However, IRKA does not require large-scale simulations of the dynamical system $H$ nor large-scale Lyapunov Equation solvers unlike Proper Orthogonal Decomposition (POD) and Balanced Trunctation (BT) respecively.
	Hence, IRKA find locally optimal solution to the $\Htwo$ approximation for less cost than competing methods that do not find optimal approximations.

	Beattie and Gugercin develop an generalization of IRKA that is realization independent of the FOM system $H$ called TF-IRKA \cite{BG12}.
	To construct the Rational Krylov spaces $\mathcal V$ and $\mathcal W$ in IRKA, a state space representation of the full-order system $H$ is required.
	Instead, TF-IRKA produces Hermite Interpolants from transfer function evaluations $H(\mu_i)$ and $H'(\mu_i)$ only via a modified Loewner-matrix approach for interpolation.

	Analogous to IRKA, the ROM transfer function
	\begin{align*}
		H_r(z) = \ve c_r^T [z \ma E_r - \ma A_r]^{-1} \ve b_r
	\end{align*}
	\noindent constructed from the Loewner-matrix state space matrices $\ma A_r, \ma E_r \in \C^{r\times r}$, $\ve b_r, \ve c_r \in \C^r$ forms a Hermite interpolant of the original transfer function $H(z)$ at the interpolation points $\{\mu_1,\ldots,\mu_r\}$ where
	\begin{align}
		\label{eq:Loewner_TFIRKA}
		\ma E_{ij} &:= \left \{ \begin{aligned}
 			&-\frac{H(\mu_i) - H(\mu_j)}{\mu_i - \mu_j}
 			\quad
 			& \mbox{if} \quad i\neq j\\
 			&-H'(\mu_i)
 			\quad
 			& \mbox{if} \quad i=j 
 			\end{aligned} \right .\nonumber \\
 		\ma A_{ij} &:= \left \{ \begin{aligned}
 			&-\frac{\mu_i H(\mu_i) - \mu_j H(\mu_j)}{\mu_i - \mu_j}
 			\quad
 			& \mbox{if} \quad i\neq j\\
 			&-[sH(s)]'|_{s=\mu_i}
 			\quad
 			& \mbox{if} \quad i=j 
 			\end{aligned} \right .\\
 		\ve b_r &:= \ve c_r^T = \begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_r) \end{bmatrix}.\nonumber
	\end{align}

	Like IRKA, TF-IRKA chooses its next interpolation points via the poles of the ROM transfer function $H_r(z)$ which are the eigenvalues of the generalized eigenvalue problem $\ve \mu^+ \leftarrow \ve -\lambda(\ma A_r, \ma E_r)$.
	When a state space representation of $H$ is available, the two algorithms are equivalent in infinite precision arithmetic.
	
%\subsection{Trust Region \texorpdfstring{$\Htwo$}{H2}}
%	[GB09]
%	\begin{align*}
%		\min_{\ve\lambda, \ve r \in \C^r} \left \| H(\cdot) - H_r(\cdot;\ve\lambda,\ve r) \right \|_{\Htwo}^2,
%		\qquad
%		H_r(z;\ve\lambda,\ve r) = \sum_{i=1}^r \frac{r_i}{z-\lambda_i}
%	\end{align*}

\subsection{QuadVF}

	Vector Fitting (VF) is an increasingly popular algorithm for rational approximation in the engineering community.
	Drma\v{c} et al.\ coupled the VF algorithm with a quadrature rule to approximate the contour integral in the $\Htwo$ norm calculation in the QuadVF algorithm \cite{DGB15}.
	The quadrature rule used is the Boyd/Clenshaw-Curtis formula \cite{B87},
	\begin{align*}
		\| H \|_\Htwo^2 \approx \sum_{j=1}^L \frac{L\pi}{(\ell+1) \sin^2 t_j} | H(\imath L \cot t_j) |^2 + \frac{\pi}{2L(\ell + 1)} ( | M_+[H] |^2 + | M_-[H] |^2 ),
	\end{align*}
	where $L>0$ is a scaling hyperparameter and $t_j = \frac{j\pi}{\ell+1}$ for $i = 1,\ldots,\ell$ and
	\begin{align*}
		M_+[H] = \lim_{\omega\to\infty} \imath \omega H(\imath \omega),
		\qquad
		M_-[H] = \lim_{\omega\to -\infty} \imath \omega H(\imath \omega).
	\end{align*}
	If $H(z)$ has the realization $H(z) = \ve c^T [z\ma I - \ma A]^{-1} \ve b$, then $M_+[H] = M_-[H] = \ve c^T \ve b$.
	Ultimately, QuadVF solves the following minimization program where the Barycentric parameters $\ve a, \ve b \in \C^r$ are chosen via Vector Fitting,
	\begin{align}
		\label{eq:quad_vf}
		\min_{\ve a, \ve b \in \C^r} 
			\left \| \begin{bmatrix} H(\imath \xi_1) \\ \vdots \\ H(\imath \xi_\ell) \\ M_+[H] \\ M_-[H] \end{bmatrix} 
			\!-\! \begin{bmatrix} H_r(\imath\xi_1;\ve a, \ve b) \\ 
				\vdots \\ H_r(\imath\xi_\ell; \ve a, \ve b) \\ M_+[H_r(\cdot; \ve a, \ve b)] \\ M_-[H_r(\cdot; \ve a, \ve b)] \end{bmatrix} 
			\right \|_{\ma W}^2,
		\quad
		H_r(z; \ve a,\! \ve b)\! =\! 
			\frac{\sum_{i=1}^r \! \frac{a_i w_i}{z - \widehat z_i} 
			\prod_{j=1}^r(z-\widehat z_j)}{\sum_{i=0}^r \! \frac{b_i w_i}{z-\widehat z_i} \prod_{j=0}^r(z-\widehat z_j)},
	\end{align}
	where $\xi_i = L\cot t_j$ and $\ma W$ is a diagonal weighting matrix from the Boyd/Clenshaw-Curtis quadrature rule.
	In practice, it is not clear what a good choice of the hyperparameter $L$ would be.
	We will revisit this challenge in the numerical results later.


==> conclusion.tex <==
\section{Conclusion}

MIMO



==> discussion_v0.tex <==
\section{Discussion}

We have introduced a new approach for computing locally optimal approximations in the $\Htwo$ norm for less cost than existing techniques.
Future work on the PH2 algorithm includes extending the approach to multiple-input/multiple-output (MIMO) dynamical systems.
The best method for initialization of both the outer loop optimization Algorithm~\ref{alg:PH2} and the nonlinear least squares formulation Algorithm~\ref{alg:lsra} remains an open question.
Additionally, PH2 is agnostic to the algorithm used to solve the NLS subproblem \eqref{eq:H2_lsra}.
A numerical study of other methods for rational approximation should be explored and compared when coupled with the PH2 algorithm.
Some examples of this could be the Accelerated Antoulas-Anderson (AAA) algorithm \cite{NST18} or Vector Fitting \cite{DGB15a,GS99}; however, currently neither method does not currently support weighted least squares.
Vector Fitting has been extended to a diagonal weighting matrix in \cite{DGB15} and perhaps could be extended further to non-diagonal weighting to accommodate the PH2 algorithm.


==> intro_v0.tex <==
\section{Introduction}
Model order reduction seeks to replace large-scale simulations in science in engineering with low-cost surrogate models, or reduced order models (ROMs) where full-scale simulations are infeasible or costly.
Construction of low-cost, high-fidelity surrogate models is expensive, hence model reduction yields its greatest impact in two computational paradigms: (1) online settings where large-scale simulations are either infeasible due to limited computational resources, and (2) many-query settings where ROM construction costs are amortized by many surrogate simulations in the process of optimization for control or parameter estimation, or high-dimensional integration for uncertainty quantification.

Model order reduction generally falls into two broad categories: (1) simulation-trained surrogate models such as Proper Orthogonal Decomposition (POD) and its many variants and extensions to nonlinear dynamics, and (2) dynamical system norm approximation, originally introduced for linear time-invariant dynamical systems and later extended to other to select nonlinear and time-varying regimes.
As model order reduction is costly, typically on the order of a full-scale simulation, considerable effort has been made to lessen or parallelize the expense.
The contribution of the paper is an algorithm that results in locally optimal approximations of single-input, single-output (SISO) linear time-invariant (LTI) dynamical systems in the $\Htwo$ norm for substantially less cost than competing methods.
Therefore, we restrict the discussion in this paper to locally optimal $\Htwo$ approximation, acknowledging its import in scientific and engineering applications.
Applications of $\Htwo$ approximation include but are not limited to Diffuse Optimal Tomography \cite{SGKCBO15,OKSG17}, structural mechanics \cite{G04,SV16}, thermal dynamics \cite{BWG08}, and optimal control \cite{G04}.

This paper compares three existing locally optimal $\Htwo$ model reduction techniques for SISO LTI model reduction: (1) the Iterative Rational Krylov Algorithm (IRKA) and a realization independent implementation called Transfer-Function IRKA (TF-IRKA), (2) a modification of the Vector Fitting algorithm, QuadVF, that includes a quadrature scheme to approximate the $\Htwo$ dynamical system norm, and (3) our algorithm, Projected $\Htwo$ (PH2), introduced in this paper.
We compare the three frameworks with numerical results for three models: (1) an infinite-dimensional heat model whose transfer function is a transcendental function, (2) a structural model of 1R module of the International Space Station, and (3) a moal model of the swing arm in a CD Player.
The results demonstrate that our approach generates comparable surrogate models for substantially less cost than the existing methodologies.

\subsection{\texorpdfstring{$\Htwo$}{H2} Optimal Model Reduction}

Necessary conditions for local $\Htwo$ optimality were introduced by Meier and Luenberger in 1967 \cite{ML67}; however, methods to find such approximations did not exist until Gugercin et al. introduced Iterative Rational Krylov Algorithm (IRKA) in 2008 \cite{GAB08}.
Until IRKA, Rational Krylov Spaces were used to build interpolatory reduced order models, however, these models were not locally optimal approximations in the $\Htwo$ norm.
Since the introduction of IRKA, $\Htwo$-based model reduction has dramatically expanded with extensions of the algorithm to a realization-independent version TF-IRKA \cite{BG12}, bilinear dynamical systems \cite{AGI16,BB12,BGG16,BB15,FG15,ZL02}, inexact computations of the Rational Krylov subspaces \cite{BG06,W12}, multiple-input/multiple-output (MIMO) dynamical systems \cite{BG12,GAB08}, parametrically dependent dynamical systems \cite{BBBG11}, linear time-periodic dynamical systems \cite{MGB18}, and cost-efficient implementations \cite{CPL16}.

\subsection{$\Htwo$ Optimal Problem Statement}

	Given a single-input, single-output (SISO) dynamical system and its transfer function,
	\begin{align}
		\label{eq:FOM}
		H : \left \{ \begin{aligned} \dve x(t) &= \ma A \ve x(t) + \ma b u(t) \\ y(t) &= \ve c^T \ve x(t) \end{aligned} \right .
		\qquad \Longrightarrow \qquad
		H(z) = \frac{\mathcal L[y](z)}{\mathcal L[u](z)} = \ve c^T [z\ma I - \ma A]^{-1} \ve b
	\end{align}
	\noindent with $\ma A \in \R^{n\times n}$, $\ve b, \ve c \in \R^n$, model reduction seeks to find a {\bf Reduced Order Model (ROM)} $H_r$,
		\begin{align*}
			H_r : \left \{ \begin{aligned} \dve x_r(t) &= \ma A_r \ve x_r(t) + \ma b_r u(t) \\ y_r(t) &= \ve c_r^T \ve x_r(t) \end{aligned} \right .
			\qquad \Longrightarrow \qquad
			H_r(z) = \frac{\mathcal L[y_r](z)}{\mathcal L[u](z)} = \ve c_r^T [z\ma I - \ma A_r]^{-1} \ve b_r,
		\end{align*}
		\noindent where $\ma A_r \in \R^{r\times r}$, $\ve b_r, \ve c_r \in \R^r$, with $r \ll n$ of substantially fewer degrees of freedom such that the outputs of the two dynamical systems approximately agree for a broad class of inputs, specifically we want $y(t) \approx y_r(t)$ for all bounded energy inputs, $\int_{-\infty}^\infty u^2(t) dt < \infty$.
	
	The $\Htwo$ Hilbert space is defined as the set of meromorphic functions that are analytic in the open right-half plane and have a bounded $\Ltwo$ norm on the contour integral along the imaginary axis,
		\begin{align*}
			\Htwo:= \left \{ f \mbox{ analytic in open right-half plane}| \int_{-\infty}^\infty |f(\imath\omega)|^2 d\omega < \infty \right \},
		\end{align*}
		
		\noindent endowed with the following norm and inner product,
		\begin{align}
			\label{eq:H2norm}
			\|f\|_{\Htwo} = \left ( \int_{-\infty}^\infty |f(\imath\omega)|^2 d\omega \right )^{1/2},
			\qquad
			\langle f,g \rangle_{\Htwo} := \frac{1}{2\pi} \int_{-\infty}^\infty \overline{f(\imath \omega)} g(\imath \omega) d\omega.
		\end{align}

		The $\Htwo$ norm bounds the $L^\infty$ norm of the error in the output:
		\begin{align*}
			\sup_{u\in L^2(0,\infty)} \frac{\|y - y_r\|_{L^\infty(0,T)}}{\| u \|_{L^2(0,\infty)}} \leq \| H - H_r \|_{\Htwo}.
		\end{align*}
		Therefore the $\Htwo$ norm functions as a performance guarantee for the error in the output $y(t) - y_r(t)$ for $t > 0$.

		The goal of $\Htwo$ optimal model reduction is to find a local minimizer $H_r$ of degree $r$ with respect to the $\Htwo$-norm of the error system,
		\begin{align}
			\label{eq:H2opt}
			\min_{\substack{H_r \in \Htwo\\ \mbox{deg}(H_r) = r}} \| H - H_r \|_{\Htwo}^2.
		\end{align}



==> lsra.tex <==
\subsection{Least Squares Rational Approximation}
Here we describe how to construct a real rational approximation of degree $(r-1,r)$
in a weighted least squares norm using standard nonlinear least squares techniques.
Our first, and most important choice, is to chose a parameterization for the rational approximation.
Assuming $H_r$ has only simple poles, a natural choice would be a pole-residue parameterization:
\begin{equation}
	H_r(z; \ve \lambda, \ve \rho) = \sum_{k=1}^n \frac{ \rho_k}{z - \lambda_k}.
\end{equation}
However, the challenge with this parameterization is enforcing the constraint that $H_r$ is real,
that $H_r(\conj z) = \conj{ H_r(z)}$.
This requires that every non-real $\lambda_k$ to have a conjugate pair in $\ve\lambda$, $\lambda_{j_k}$, and that for these values $\rho_k = \conj \rho_{j_k}$, and that if $\lambda_k$ is real, that $\rho_k$ is also real.
%Using this parameterization with the real constraint is difficult
%as when one of the $\lambda_k$ goes from being complex to real,
%the least squares problem is not differentiable.
Instead, our approach is to parameterize $H_r$ using a partial fraction expansion in quadratic terms:
\begin{equation}\label{eq:quadpartial}
	H_r(z; \ve a, \ve b) =
		\sum_{k=1}^{\lfloor r/2 \rfloor} 
			\frac{ a_{2k} z + a_{2k-1}}{ z^2 + b_{2k} z + b_{2k-1}};
	\quad
	\ve a, \ve b \in \R^r
\end{equation}
where we assume that $r$ is even.
Then since $\ve a$ and $\ve b$ are both real, $H_r(z;\ve a, \ve b)$ is a real rational function.
To convert back to poles and residues, we can simply use the quadratic formula to determine 
the roots of denominator polynomials above.

To then solve the nonlinear least squares problem:
\begin{equation}\label{eq:H2_lsra}
	\minimize_{\ve a, \ve b\in \R^r}
		\left\|
			\ma M(\mu)^{-1/2}
			\left(
				\begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_n)\end{bmatrix}
				-
				\begin{bmatrix} H_r(\mu_1; \ve a, \ve b) \\ \vdots \\ H_r(\mu_n; \ve a, \ve b) \end{bmatrix}
			\right)	
		\right\|_2,
\end{equation}
we exploit the fact that the parameters $\ve a$ appear linearly 
and use \emph{Variable Projection} (VARPRO)~\cite{GP73} reduce~\cref{eq:H2_lsra}
to an optimization problem over $\ve b$ alone.
\Cref{alg:lsra} gives expressions for the (complex) residual and Jacobian for this problem
and couples it with a simple Gauss-Newton iteration with a backtracking line search. 

\input{alg_lsra} 




==> pnls.tex <==
\section{Projected Nonlinear Least Squares\label{sec:pnls}}

	Demmel developed an algorithm to compute the Singular Value Decomposition (SVD) of an ill-conditioned Cauchy matrix $\ma M(\ve \mu)$ with high relative accuracy \cite{D00}:
	\begin{align*}
		\mbox{svd}(\ma M(\ve\mu)) = \mbox{svd} \left (\begin{bmatrix}
			\frac{1}{\mu_1 + \overline{\mu_1}} & \hdots & \frac{1}{\mu_1 + \overline{\mu_n}} \\
			\vdots & \ddots & \vdots \\
			\frac{1}{\mu_n + \overline{\mu_1}} & \hdots & \frac{1}{\mu_n + \overline{\mu_n}}
		\end{bmatrix} \right ) = \ma U \ma \Sigma \ma U^*, \qquad \ma M(\ve \mu)^{1/2} = \ma U \ma \Sigma^{1/2}.
	\end{align*}
	
	Instead of the solving the original formulation \eqref{eq:H2opt}, we solve instead a nearby problem written as a nonlinear least squares problem,
	\begin{align}
		\label{eq:H2lsq}
		\min_{\substack{H_r \in \Htwo\\ \mbox{deg}(H_r) = r}} \| P_{\ve\mu} (H - H_r) \|_{\Htwo}
		= \left \| \ma M(\ve \mu)^{-1/2} \left ( \begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_n) \end{bmatrix} - \begin{bmatrix} H_r(\mu_1) \\ \vdots \\ H_r(\mu_n) \end{bmatrix} \right ) \right \|_2^2.
	\end{align}
	
	Clearly, the choice of $\ve \mu$ is critical to how nearby the two problems \eqref{eq:H2opt} and \eqref{eq:H2lsq} are.
	Hence, we propose an algorithm that iteratively augments the sample selection $\ve \mu$ to approximate necessary conditions for optimality.

	The choice of parameterization for the ROM $H_r$ matters here. We implement a pole-residue expansion of the ROM,
	\begin{align*}
		H_r(z;\ve\lambda) = \sum_{i=1}^r \frac{r_i}{z-\lambda_i}.
	\end{align*}


Note that the second step in Algorithm~\ref{alg:PH2} requires an initialization of the poles $\ve \lambda \in \C^r$.
We consider two choices for initialization: (1) initialize with the poles of previous iteration of the nonlinear least squares subproblem \eqref{eq:H2_lsra}, or (2) initialize with the poles from the Accelerated Antoulas-Anderson (AAA) algorithm \cite{NST18}.
Based on the authors' experience, both choices are effective but neither consistently outperforms the other.
Hence, because we consider a large-scale setting where the dominant cost is the function evaluations $\{H(\mu_1),\ldots,H(\mu_n)\}$, the inner loop optimization of Algorithm~\ref{alg:lsra} is relatively inexpensive and we run it with both choices of initialization, using the result that yields the least residual of the least squares program.



==> pnls_v0.tex <==
\section{Projected Nonlinear Least Squares\label{sec:pnls}}
	The $\Htwo$ Hilbert space forms a reproducing kernel Hilbert space via Residue Calculus,
	\begin{align*}
		H(\mu) = \langle v_\mu, H \rangle_{\Htwo},
		\qquad
		v_\mu(z) := (z + \overline{\mu})^{-1}.
	\end{align*}
		The result follows immediately from the Cauchy Integral Formula:
	\begin{align*}
		\langle v_\mu, H \rangle_\Htwo
		&= \frac{1}{2\pi} \int_{-\infty}^\infty \conj{v_\mu(i\omega)} H(i\omega) d\omega
		= \frac{1}{2\pi} \int_{-\infty}^\infty \frac{1}{-i\omega+\mu} H(i\omega) d\omega\\
		&= \frac{-1}{2\pi} \int_{-\infty}^\infty \frac{1}{i\omega - \mu} H(i\omega) d\omega
		= \frac{-\imath}{2\pi} \lim_{R\to\infty} \int_{D_R} \frac{1}{z - \mu} H(z) dz
		= H(\mu),
	\end{align*}
	\noindent where $D_R$ denotes the semicircle along the imaginary axis with and the right-half plane. As the contour integral is evaluated counter-clockwise, $z = -\imath\omega$ on the imaginary axis implies that $dz = -\imath d\omega$.
	
	Our goal is to convert the $\Htwo$ optimization problem \eqref{eq:H2opt} into a nearby problem of the nonlinear least squares structure.
	We accomplish this by projecting the error system $H - H_r$ onto a finite dimensional subspace of $\Htwo$ spanned by the set of primitives $\{v_{\mu_1}, \ldots, v_{\mu_n}\}$ via an operator $V(\ve \mu): \C^n \to \mbox{span}\{ v_{\mu_1}, \ldots, v_{\mu_n} \}$ who adjoint is the sampling operator $V(\ve \mu)^* : \Htwo \to \C^n$,
	\begin{align*}
		[V(\ve \mu)\ve c](z) = \sum_{j=1}^n \frac{c_j}{z + \overline{\mu_j}},
		\qquad
		V(\ve \mu)^* H
		= \begin{bmatrix} \langle v_{\mu_1}, H \rangle_\Htwo \\ \vdots \\ \langle v_{\mu_n}, H \rangle_\Htwo \end{bmatrix}
		= \begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_n) \end{bmatrix}.
	\end{align*}
	Then $V(\ve\mu)$ and $V(\ve\mu)^*$ satisfy the adjoint identity $\langle V(\ve\mu)\ve c, H \rangle_{\Htwo} = \langle \ve c, V(\ve\mu)^* H \rangle_{\C^n}$.

	Define the orthogonal projection $P_{\ve \mu} : \Htwo \to \mbox{span}\{v_{\mu_1},\ldots,v_{\mu_n}\}$:
	\begin{align*}
		P_{\ve \mu} &:= V(\ve \mu) \ma M(\ve \mu)^{-1} V(\ve \mu)^*,
		\qquad
		\ma M(\ve \mu)_{ij} := [V(\ve \mu)^* V(\ve \mu)]_{ij} = v_{\mu_j}(\mu_i) = (\mu_i + \overline{\mu_j})^{-1}.
	\end{align*}
	Then $V(\ve \mu) \ma M(\ve \mu)^{-1/2}: \C^n \to \mbox{span}\{v_{\mu_1},\ldots,v_{\mu_n}\}$ is a unitary mapping and therefore
	\begin{align*}
		\| H - H_r \|_\Htwo^2 \geq \| P_{\ve\mu} ( H - H_r) \|_\Htwo^2 = \left \| \ma M(\ve \mu)^{-1/2} \left ( \begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_n) \end{bmatrix} - \begin{bmatrix} H_r(\mu_1) \\ \vdots \\ H_r(\mu_n) \end{bmatrix} \right ) \right \|_2^2.
	\end{align*}

	Demmel developed an algorithm to compute the Singular Value Decomposition (SVD) of an ill-conditioned Cauchy matrix $\ma M(\ve \mu)$ with high relative accuracy \cite{D00}:
	\begin{align*}
		\mbox{svd}(\ma M(\ve\mu)) = \mbox{svd} \left (\begin{bmatrix}
			\frac{1}{\mu_1 + \overline{\mu_1}} & \hdots & \frac{1}{\mu_1 + \overline{\mu_n}} \\
			\vdots & \ddots & \vdots \\
			\frac{1}{\mu_n + \overline{\mu_1}} & \hdots & \frac{1}{\mu_n + \overline{\mu_n}}
		\end{bmatrix} \right ) = \ma U \ma \Sigma \ma U^*, \qquad \ma M(\ve \mu)^{1/2} = \ma U \ma \Sigma^{1/2}.
	\end{align*}
	
	Instead of the solving the original formulation \eqref{eq:H2opt}, we solve instead a nearby problem written as a nonlinear least squares problem,
	\begin{align}
		\label{eq:H2lsq}
		\min_{\substack{H_r \in \Htwo\\ \mbox{deg}(H_r) = r}} \| P_{\ve\mu} (H - H_r) \|_{\Htwo}
		= \left \| \ma M(\ve \mu)^{-1/2} \left ( \begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_n) \end{bmatrix} - \begin{bmatrix} H_r(\mu_1) \\ \vdots \\ H_r(\mu_n) \end{bmatrix} \right ) \right \|_2^2.
	\end{align}
	
	Clearly, the choice of $\ve \mu$ is critical to how nearby the two problems \eqref{eq:H2opt} and \eqref{eq:H2lsq} are.
	Hence, we propose an algorithm that iteratively augments the sample selection $\ve \mu$ to approximate necessary conditions for optimality.

	The choice of parameterization for the ROM $H_r$ matters here. We implement a pole-residue expansion of the ROM,
	\begin{align*}
		H_r(z;\ve\lambda) = \sum_{i=1}^r \frac{r_i}{z-\lambda_i}.
	\end{align*}

	\begin{algorithm}
	\begin{minipage}{\linewidth}
	\begin{algorithm2e}[H]
		\Input{$H \in \Htwo$ and $2r$ initial samples $\{\mu_1,\ldots,\mu_{2r}\}$}
		\Output{ROM $H_r \in \Htwo$}
		\For{$n=2r,2r+2,2r+4,\ldots$}{
			Solve the projected nonlinear least squares program:
			$H_r = \argmin_{\ve\lambda, \ve r \in \C^n} \left \| \begin{bmatrix} H(\mu_1) \\ \vdots \\ H(\mu_n) \end{bmatrix} - \begin{bmatrix} H_r(\mu_1;\ve\lambda,\ve r) \\ \vdots \\ H_r(\mu_n;\ve\lambda,\ve r) \end{bmatrix} \right \|_{\ma M(\ve \mu)^{-1}}^2$\\
			via Algorithm~\ref{alg:lsra}\;
			Compute the poles of $H_r$:
			$\{\lambda_i\}_{i=1}^r \leftarrow \ve\lambda(H_r)$\;
			Determine the largest subspace angle:
			$\lambda^* = \argmax_{\lambda \in \{\lambda_i\}_{i=1}^r} \measuredangle	(\mbox{span}\{v_{\mu_1},\ldots,v_{\mu_n}\}, \mbox{span}\{ -\lambda, -\overline{\lambda} \})$\;
			Augment the subspace:
			$\{\mu_i\}_{i=1}^{n+2} \leftarrow \{\mu_1,\ldots,\mu_n,-\lambda^*, -\overline{\lambda^*} \}$\;
		}
\end{algorithm2e}
\caption{Projected Nonlinear Least Squares for $\Htwo$ (PH2)}
\label{alg:PH2}
\end{minipage}
\end{algorithm}

Note that the second step in Algorithm~\ref{alg:PH2} requires an initialization of the poles $\ve \lambda \in \C^r$.
We consider two choices for initialization: (1) initialize with the poles of previous iteration of the nonlinear least squares subproblem \eqref{eq:H2_lsra}, or (2) initialize with the poles from the Accelerated Antoulas-Anderson (AAA) algorithm \cite{NST18}.
Based on the authors' experience, both choices are effective but neither consistently outperforms the other.
Hence, because we consider a large-scale setting where the dominant cost is the function evaluations $\{H(\mu_1),\ldots,H(\mu_n)\}$, the inner loop optimization of Algorithm~\ref{alg:lsra} is relatively inexpensive and we run it with both choices of initialization, using the result that yields the least residual of the least squares program.

\subsection{Meier-Luenberger Necessary Conditions for Optimality}

If the sample points $\mu$ cluster near the reflection of the pole of the primitive $v_{-\conj{\lambda}}$, then the primitive can pass through the projection in the limit.

\begin{theorem}
	\label{thm:conv}
	Suppose $\lbrace \mu_k \rbrace_{k=1}^\infty$ is a sequence of samples generated by \cref{alg:LSRA}
	with $r$ distinct limit points $\lbrace \widehat \mu_k \rbrace_{k=1}^r$.
	Moreover, assume that for each convergent subsequence converge to but do not intersect an element in $\{\widehat \mu_k\}_{k=1}^r$.
	If $H_r^{(N)}$ is the rational approximation satisfying the first order necessary conditions
	for the projected problem,
	then for any $\epsilon > 0$ there exists an $\widehat{N}$ such that 
	the Meier-Luenberger conditions are approximately satisfied for all $N> \widehat{N}$; i.e., 
	\begin{align}
		|\langle u, H - H_r^{(N)}\rangle_\Htwo| &< \epsilon 
		\quad \forall u \in \hset W :=\lbrace v_{\widehat\mu_k}\rbrace_{k=1}^r \cup \lbrace v_{\widehat \mu_k}' \rbrace_{k=1}^r
		\quad \forall N > \widehat{N}.
	\end{align}
\end{theorem}

A proof of this theorem is included in the appendix of this document.

\input{lsra}

